Fine-Tuning Pre-trained Language Model with Weak Supervision: A Contrastive-Regularized Self-Training Approach

Fine-tuned pre-trained language models (LMs) have achieved enormous success in many natural language processing (NLP) tasks, but they still require excessive labeled data in the fine-tuning stage. We study the problem of fine-tuning pre-trained LMs using only weak supervision, without any labeled data. This problem is challenging because the high capacity of LMs makes them prone to overfitting the noisy labels generated by weak supervision. To address this problem, we develop a contrastive self-training framework, COSINE, to enable fine-tuning LMs with weak supervision. Underpinned by contrastive regularization and confidence-based reweighting, this contrastive self-training framework can gradually improve model fitting while effectively suppressing error propagation. Experiments on sequence, token, and sentence pair classification tasks show that our model outperforms the strongest baseline by large margins on 7 benchmarks in 6 tasks, and achieves competitive performance with fully-supervised fine-tuning methods.

==> 4.1reweight.tex <==
\noindent \textbf{Uncertainty-driven sample reweighting.}
While the generated pseudo-labels enable the model to update periodically, directly training with these labels is prone to error propagation caused by wrongly labelled data with high uncertainties. To alleviate this, we 
reweight samples based on the confidence of pseudo-labels during self-training. In our problem, we use \emph{entropy} as a measure of uncertainty. For each sample $x$ with soft pseudo-label $\tilde{\by}$, we assign $x$ with a weight $\omega$ defined by \yue{I think we can change `confidence' to uncertainty}
\begin{equation}
\omega=1-\frac{H\left({\tilde{\by}}\right)}{\log (C)},
\label{eq:rewconf}
\end{equation}
where $H(\tilde{\by}) = -\sum_{i=1}^{C}\tilde{\by}_i \log{\tilde{\by}_i}$ is the entropy of $\tilde{\by}$ with $0 \leq H(\tilde{\by}) \leq \log{C}$. If the data uncertainty is high, then $H(\tilde{\by})$ is also large, thus $\omega$ will be low. To further suppress the low-confidence samples, we use a threshold $\xi$ to select high confidence examples from each batch $\cB$ as 
\begin{equation}
\cC = \{x| \omega(x) \geq \xi\}.
\label{eq:C}
\end{equation}
% Finally, the weight $\omega$ is calculated as  
% \begin{equation}
% %  \setlength{\abovedisplayskip}{0.1pt}
% % \setlength{\belowdisplayskip}{0.15pt}
% \omega=\left\{\begin{array}{ll}
% \omega & \text { if } \omega \geq \xi \\
% 0 & \text { else } 
% \end{array}\right..
% \label{eq:threshw}
% \end{equation}
Then we can rewrite the classification loss  as 
\begin{equation}
%  \setlength{\abovedisplayskip}{0.1pt}
% \setlength{\belowdisplayskip}{0.15pt}
\mathcal{L}_c(\theta, \tilde{\by}) = \frac{1}{|\cC|}\sum_{x \in \cC} \omega_i \ell(\hat{f}(x ; \theta), \tilde{\by}),
\label{eq:newloss}
\end{equation}
where $\omega_i$ is calculated via Eq.~\eqref{eq:rewconf} and $\ell(\cdot,\cdot)$ is the KL-divergence loss defined in Eq.~\eqref{eq:kl}.% with $\tilde{y}_{i}$.

==> 4.2confreg.tex <==
\noindent \textbf{Confidence regularization.}
The sample reweighting approach above promotes high confidence sample during self-training. To % further prevent over confidence -
%To further prevent the model from aggressively updating and 
prevent the over-confident predictions, we add confidence regularization on models in during self-training.
Specifically, for each sample $x$, we regularize the model ${f}(\cdot;\theta)$  by an smoothness encouraging term based on the model prediction as 
\begin{equation}
\mathcal{R}_2(\theta) =  \frac{1}{|\cC|} \sum_{x \in \cC} \mathcal{D}_{\text{KL}}\left(\mathbf{u} \| {f}(x; \theta)\right),
\label{eq:confreg}
\end{equation}
where $\mathcal{D}_{\text{KL}}$ is the Kullback--Leibler divergence as Eq.~\eqref{eq:kldef} and $\mathbf{u}$ is the uniform vector.

